Imitating Graph-Based Planning with Goal-Conditioned Policies

Recently, graph-based planning algorithms have gained much attention to solve goal-conditioned reinforcement learning (RL) tasks: they provide a sequence of subgoals to reach the target-goal, and the agents learn to execute subgoal-conditioned policies. However, the sample-efficiency of such RL schemes still remains a challenge, particularly for long-horizon tasks. To address this issue, we present a simple yet effective self-imitation scheme which distills a subgoal-conditioned policy into the target-goal-conditioned policy. Our intuition here is that to reach a target-goal, an agent should pass through a subgoal, so target-goal- and subgoal- conditioned policies should be similar to each other. We also propose a novel scheme of stochastically skipping executed subgoals in a planned path, which further improves performance. Unlike prior methods that only utilize graph-based planning in an execution phase, our method transfers knowledge from a planner along with a graph into policy learning. We empirically show that our method can significantly boost the sample-efficiency of the existing goal-conditioned RL methods under various long-horizon control tasks.

==> algorithm/algo.tex <==
\begin{algorithm}[tb]
   \caption{Self-Imitating Goal-Conditioned Policies}
   \label{alg:algo}
\begin{algorithmic}
\STATE {\bfseries Input}: Number of training episodes $N$, horizon $H$
\STATE Initialize replay buffer $\mathcal{B} \leftarrow \varnothing$.
\STATE Initialize the parameters of goal-conditioned policy $\pi_{\theta}$.
\FOR{$n=1, 2, 3, \ldots N$}
\STATE Sample a target goal $g$ and an initial state $s_{0}$.
    \FOR{$t=1, 2, 3, \ldots H$}
    \STATE Build a graph $G = (L, E, d)$ using $\mathcal{B}$.
    \STATE Find the shortest subgoal-path $\tau_{g}$ from $s_{t}$ to $g$.
    \STATE \junsu{Find a desired subgoal $l^{*}$ via Algorithm~\ref{alg:skip}.}
    \STATE Collect a transition $(s_{t}, a_{t}, r_{t})$ using $\pi_{\theta} (s_{t}, l^{*})$.
    \STATE Store the transition and the planned path $\tau_{g}$ in $\mathcal{B}$.
    \STATE Train a policy $\pi_{\theta}$  with $\mathcal{B}$ according to \junsu{Equation} \ref{eq:total_loss}.
    \ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> figure/1_concept_legacy.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}{0.495\textwidth}
    \includegraphics[width=1\linewidth]{figure/concept_a.pdf}
    \caption{Self-imitation for training}
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}{0.495\textwidth}
    \includegraphics[width=1\linewidth]{figure/concept_b.pdf}
    \caption{Subgoal skipping for execution}
    \end{subfigure}
    \caption{Illustration of \Algname (\ALGname). The key ingredient of \ALGname is twofold: (a) self-imitation via planning and (b) subgoal skipping. For (a), we distill a subgoal-conditioned policy into the target-conditioned policy via our proposed loss term $\mathcal{L}_{\mathtt{\ALGname}}$. For (b), when we execute a policy along with a graph-based planning, we provide a subgoal depending on the strength of a current policy, measured by our proposed loss term $\mathcal{L}_{\mathtt{\ALGname}}$.}
    \label{fig:concept}
\end{figure*}

==> figure/3_additional_comparative.tex <==
\begin{figure}[t!]
\begin{minipage}[b]{.45\textwidth}
\centering
\includegraphics[width=1\textwidth]{NeurIPS22/figure/L3P+PIG.pdf}
\caption{This is caption of test1.\newline\newline}
\label{fig:HOG_resolution}
\end{minipage}
\hfill
\begin{minipage}[b]{.45\textwidth}
\centering
\includegraphics[width=1\textwidth]{NeurIPS22/figure/U-shaped AntMaze Planner.pdf}
\caption{Test time success rate of \ALGname and MSS on U-shaped Ant Maze environment. The \textbf{w/o planner} means that planner is not used at test time, so a goal is directly fed into the policy instead of a subgoal. Intriguingly, we find that MSS + \ALGname without a planner can achieve competitive performance to MSS and MSS + \ALGname that utilize a planner.}
\label{fig:planner}
\end{minipage}
\end{figure}


==> figure/3_l3p.tex <==
% \begin{figure*}[t]
\begin{wrapfigure}{r}{0.4\linewidth}
    \vspace{-.2in}
    \centering
    \includegraphics[width=1.0\linewidth]{NeurIPS22/figure/L3P+PIG.pdf}
    \caption{Test time success rate of \ALGname on top of varying planning-based GCRL method: MSS and L3P in U-shaped AntMaze.
    }
    \vspace{-.2in}
    \label{fig:l3p}
\end{wrapfigure}
% \end{figure*}


==> figure/3_support_results.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}{0.33\textwidth}
    \includegraphics[width=1.0\linewidth]{figure/BC ablation.pdf}
    \caption{vs BC}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
    \includegraphics[width=1.0\linewidth]{example-image-a}
    \caption{vs HIGL}
    \end{subfigure}
    \caption{Additional experimental results that demonstrate the effectiveness of \ALGname. L-shaped AntMaze}
    \label{fig:support}
\end{figure*}
